Editing Conceptual Knowledge for Large Language Models

Recently, there has been a growing interest in knowledge editing for Large Language Models (LLMs). Current approaches and evaluations merely explore the instance-level editing, while whether LLMs possess the capability to modify concepts remains unclear. This paper pioneers the investigation of editing conceptual knowledge for LLMs, by constructing a novel benchmark dataset ConceptEdit and establishing a suite of new metrics for evaluation. The experimental results reveal that, although existing editing methods can efficiently modify concept-level definition to some extent, they also have the potential to distort the related instantial knowledge in LLMs, leading to poor performance. We anticipate this can inspire further progress in better understanding LLMs. Our project homepage is available at https://zjunlp.github.io/project/ConceptEdit.

==> sections/tab/data_compare.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|c|}
\hline
ConceptEdit &  & CounterFact &  \\ \hline
id & 1 & case\_id & 8 \\ \hline
concept\_name & military person & prompt & What is the twin city of Wellington? It is \\ \hline
concept\_def & those who serve as part of an organized armed military force & target\_new & Sheffield \\ \hline
top\_superclass & species & ground\_truth & Sydney \\ \hline
instances & {[}"Ronald Reid-Daly", "Charles Augustus   Hilton","27th Indiana Infantry Regiment","Spartaco   Schergat", "Charles Corcoran", "Franois Claude Amour,   marquis de Bouill", "Clyde A. Vaughn", "Earle   Wheeler", "Joe McCarthy", "Central African Republic Civil   War", "Andrew Mathews", "Nikolaus Heilmann",   "Ahmed Abdel Rahman Nasser", "Reed McKinley Chambers",   "Wallace Lawler", "Clarence Tan", "Louis Charles   mile Gibon-Guilhem", "Manshuk Mametova", "Moshe   Tzadok", "John F. G. Howe"{]} & rephrase\_prompt & People in Wellington's twin city speak the language of \\ \hline
QID & Q47064 & locality\_prompt & What is the twin city of Chicago? It is \\ \hline
module\_intra & \{"replace\_from\_concept": "jockey", "replace\_def":     "someone who rides horses in horse racing or steeplechase racing"     \} & locality\_ground\_truth & Sydney \\ \hline
module\_inter & \{"replace\_from\_concept":"settlement","replace\_def":   "place of any size, in which people live"\} &  &  \\ \hline
locality\_prompt & The definition of bacteria is &  &  \\ \hline
locality\_answer & domain of micro-organisms &  &  \\ \hline
\end{tabular}
\end{table}
